Emerging Synergies in Causality and Deep Generative Models: A Survey

In the field of artificial intelligence (AI), the quest to understand and model data-generating processes (DGPs) is of paramount importance. Deep generative models (DGMs) have proven adept in capturing complex data distributions but often fall short in generalization and interpretability. On the other hand, causality offers a structured lens to comprehend the mechanisms driving data generation and highlights the causal-effect dynamics inherent in these processes. While causality excels in interpretability and the ability to extrapolate, it grapples with intricacies of high-dimensional spaces. Recognizing the synergistic potential, we delve into the confluence of causality and DGMs. We elucidate the integration of causal principles within DGMs, investigate causal identification using DGMs, and navigate an emerging research frontier of causality in large-scale generative models, particularly generative large language models (LLMs). We offer insights into methodologies, highlight open challenges, and suggest future directions, positioning our comprehensive review as an essential guide in this swiftly emerging and evolving area.

==> figures/fig_paper_structure.tex <==
\begin{forest}
  for tree={
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=left,
  font=\normalsize,
  rectangle,
  draw,
  rounded corners,align=center,
  minimum width=2.5em,
  inner xsep=4pt,
  inner ysep=1pt,
  },
  where level=1{text width=5em,fill=blue!10}{},
  where level=2{text width=5em,font=\normalsize,fill=pink!30}{},
  where level=3{font=\normalsize,yshift=0.26pt,fill=yellow!20}{},
  [Emerging Synergies in Causality\\ and Deep Generative Models,fill=green!20
    [
        {\S \ref{241725040005} Background}, text width=6.5em, fill=blue!10
        [
        {Causality},text width=4em,fill=pink!30
        ]
        [
        Deep Generative Models,text width=11em,fill=pink!30
        ]
    ]
    [
        \S \ref{971699495725} Integrating Causal Principles in DGMs, text width=19em, fill=blue!10
        [
        Rationale for Causal Integration in DGMs,text width=19em, fill=pink!30
        ]
        [
        Setting the Stage for Causal Generative Models,text width=21.3em,fill=pink!30
        ]
        [
        Classifying Methods of Causal Integration,text width=19em,fill=pink!30
        ]
    ]
    [
        \S \ref{776815666820} Identifying Causality via DGMs,text width=15.6em, fill=blue!10
        [
        Causal Discovery through DGMs,text width=15em,fill=pink!30
        ]
        [
        Counterfactual Inference Leveraging DGMs,text width=20.0em,fill=pink!30
        ]
        [
        Causal Representation Learning using DGMs,text width=20.6em,fill=pink!30
        ]    
    ]
    [
        \parbox{17em}{\S \ref{605156580006} Exploring Causality within Large-scale DGMs: An Emerging Frontier},text width=17em, fill=blue!10
        [
        \parbox{22em}{Assessing Causal Capabilities in Current LLMs: Memorization or Reasoning?},text width=22em,fill=pink!30
        ]
        [
        Advancing Causal Research Through LLMs,text width=20em,fill=pink!30
        ]  
    ]
    [
        {\S \ref{471209836872} Trustworthy Properties},text width=12em, fill=blue!10
        [
        {Generalization},text width=7em,fill=pink!30
        ]
        [
        {Fairness},text width=4em,fill=pink!30
        ]  
        [
        {Interpretability},text width=7em,fill=pink!30
        ] 
    ]
    [
        {\S \ref{591853874791} Applications},text width=7em, fill=blue!10
        [
        {Computer Vision},text width=8em,fill=pink!30
        ]
        [
        {Health Science},text width=6.6em,fill=pink!30
        ]  
        [
        {Social Science},text width=6.6em,fill=pink!30
        ] 
    ]
    [
        {\S \ref{996252365804} Discussion},text width=6.6em, fill=blue!10
        [
        Understanding generated counterfactuals,text width=19em,fill=pink!30
        ]
        [
        Challenges with Large-scale Causal Graphs,text width=20em,fill=pink!30
        ]  
        [
        Incorporating Causal Discovery and Representation Learning,text width=28em,fill=pink!30
        ]
        [
        Causal Learning within Large-scale Generative Models,text width=24.6em,fill=pink!30
        ] 
    ]
]
\end{forest}

        

==> figures/fig_tree.tex <==
\begin{forest}
  for tree={
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=left,
  font=\small,
  rectangle,
  draw,
  rounded corners,align=left,
  minimum width=2.5em,
  inner xsep=4pt,
  inner ysep=1pt,
  },
  where level=1{text width=5em,fill=blue!10}{},
  where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
  where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
  [Interplay of \\ cauaslity and DGMs,fill=green!20
        [Causality Identification\\ via DGMs (\S ~\ref{776815666820}),text width=10em
            [Causality Discovery,text width=8em
            ]
            [Causal Representation Learning,text width=12em 
            ]
        ]
        [Emebdding Causal\\ Principles in DGMs (\S ~\ref{971699495725}),text width=12em
          [GANs-Based,text width=8.5em
            [
            CausalGAN~\cite{Kocaoglu2018CausalGANLC}/CGN~\cite{Sauer2021CounterfactualGN}/CausalTGAN~\cite{Wen2021CausalTGANGT}/CFGAN~\cite{Xu2019AchievingCF}/DECAF~\cite{Breugel2021DECAFGF}/DEAR~\cite{shen2022weakly}/GenInt~\cite{Mao2021GenerativeIF}/PKD~\cite{Feng2022PrincipledKE}
            ]
          ]
          [VAEs-Based, text width=8.5em
              [
              CausalVAE~\cite{Yang2021CausalVAEDR}
              ]
          ]
          [Diffusion-Based, text width=8.5em
              [
              Diff-SCM~\cite{Sanchez2022DiffusionCM}/DCM~\cite{chao2023interventional}/CDPM~\cite{Sanchez2022WhatIH}
              ]
          ]
        ]
        [An Emergent Frontier involving\\ Causality with Large-scale\\ Generative Models (\S ~\ref{605156580006}),text width=14em
          [Causality as Language\\ Comprehension,text width=9em
            ]
           [
           Causality as Knowledge, text width=9em
           ]
           [Causality as Reasoning, text width=9em]
        ]
    ]
\end{forest}

==> secs/sec_method.tex <==
\subsection{GANs-Based Models}
% Generative Adversarial Networks (GANs) \cite{Goodfellow2014GenerativeAN} estimate generative models by an adversarial process, including a generator network that captures empirical distribution and a discriminator network that classifies real observational or fake generated samples.
% as shown on the left in Figure \ref{925818866720}. 
% GANs currently hold the state-of-the-art on most generation tasks due to eliminating the Markov chains and avoiding unrolled approximate inference. 
Although GANs \cite{Mirza2014ConditionalGA, Goodfellow2014GenerativeAN} have achieved state-of-the-art performance on many generation tasks and
several studies have designed controllable data generation \cite{wang2022controllable}, i.e., InfoGAN \cite{Chen2016InfoGANIR}, issues in Section \ref{981500436031} still exist. 
In an attempt to improve controllability and interpretability of GAN-generated data, some studies have combined GANs with causality by either translating SCMs into GAN architectures or enforcing causal mechanisms in the generative strategies of GANs.

\subsubsection{Translate SCMs into GANs}

Specific approaches explicitly convert SCMs into the architecture of GANs, including the generator, the prior for latent variables and auxiliary internal representations.    

\begin{figure}[!hb]
    \centering
    \includegraphics[width=\linewidth]{figures/gan_generator_structure.pdf} 
    \caption{\protect\cite{Kocaoglu2018CausalGANLC} illustrate the process of translating an SCM into the structure of a generator architecture  using a simplified causal graph $\{A\rightarrow X \leftarrow B\}$.}
    \label{925818866720}
\end{figure}
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{Snipaste_2022-11-08_17-59-00.jpg} 
%     \caption{The assumed causal graph in CausalGAN \protect\cite{Kocaoglu2018CausalGANLC} for a subset in the CelebA dataset.}
%     \label{925818866720}
% \end{figure}

\paragraph{\textbf{SCMs as a Generator in GANs}}
\cite{Kocaoglu2018CausalGANLC} introduce CausalGAN, the first work combining GANs with SCMs.
In particular, the generator architecture in CausalGAN is structured based on an assumed causal graph illustrated in Figure \ref{040922319451}, and we present a simplified illustration in Figure \ref{925818866720}.  
For example, there are two attributes named ${Gender}$ and ${Mustache}$ in CelebA dataset \cite{liu2015faceattributes}. 
Obviously, a causal relationship exists with $\{Age \rightarrow Mustache \leftarrow Gender\}$ in Figure \ref{040922319451}. 
Supposing that we sample from a conditional distribution of $P(\cdot \vert Mustache=1)$, then we attain data examples only with $\{Gender=Male\}$ 
since there is a causal factor of $\{Gender=Male\}$ that induces $\{Mustache=1\}$.
However, causality allows us to sample from different distributions when performing interventions on causal variables in an SCM. 
As Figure \ref{040922319451} shows, we intervene on the $Mustache$ variable by replacing the structural assignments on $Mustache$ variable with a new mechanism, which the simplest mechanism is atomic intervention when $Mustache$ is one or zero. 
In this way, we cut off the causal relationships from $\{Age, Gender\}$ to $Mustache$, and the causal effects disappear. 
Then specific samples, which are unseen in observables, are expected to generate, i.e., a female with mustache or a child with mustache, able to extrapolate current training distributions.  
In such a manner, they extend beyond previous conditional generations by exploiting causal relationships among attribute variables. 
Besides, CausalGAN provides a theoretical guarantee for the correctness of sampling from interventional distributions but is only limited to binary attributes. Although CausalGAN contributes to more creative models that yield samples different from training ones in multiple ways, there is no further demonstration of the benefits of the generated data for subsequent tasks \cite{Kocaoglu2018CausalGANLC}. 
% which enables to sample not only from observational data but also interventional distributions. 
% Causal lens induced in CausalGAN contribute to vanilla GAN \cite{Goodfellow2014GenerativeAN} and BEGAN \cite{Berthelot2017BEGANBE} since they can produce samples that are different from training samples, a.k.a, generating out-of-distribution instances. 
% since there can't be such instances of $\{Gender=Female, Mustache=1\}$ in the training distribution. 


% \cite{Sauer2021CounterfactualGN} consider decomposing the image generation process into three \textit{independent mechanisms} (IMs) \cite{peters2017elements} controlling factors of variation, including shape, texture and background. 
Similar to CausalGAN, the counterfactual generative network (CGN) \cite{Sauer2021CounterfactualGN} also induces the proposed SCMs into the architecture of the generator network, controlling factors of variation, including shape, texture and background. 
% With these three IMs, this work could produce samples from combinations of factors of variation, a.k.a. counterfactual samples. 
Unlike CausalGAN, CGN aims to obtain more robust and interpretable classifiers and prevent classifiers from learning shortcuts \cite{Geirhos2020ShortcutLI}. 
% They design such counterfactual generative networks and then generate counterfactual samples as data augmentation to improve downstream classification tasks.
They regard counterfactual samples generated from CGN for data augmentation and investigate whether these counterfactual images enable invariant classifiers. 
Empirical evaluations confirm that counterfactual data augmentation leads to invariant classifiers on MNIST. 
However, the gap to a fully invariant classifier still exists on ImageNet-9.


In a scenario of tabular data generation, 
% previous GANs-based works do not consider the relationship between inter-variables. 
% Thus, 
\cite{Wen2021CausalTGANGT} propose designing a causally-aware generator architecture in GANs by modeling predefined causal relationships.  
% Analogously, \cite{Xu2019AchievingCF} and \cite{Breugel2021DECAFGF} also arrange the generator structure obeying a given causal graph. 
Unlike previous studies, \cite{Xu2019AchievingCF} and \cite{Breugel2021DECAFGF} start from a fairness perspective.
\cite{Xu2019AchievingCF} build a causal fairness-aware GAN (CFGAN) that enforces various causal fairness principles, such as total effect, direct or indirect discrimination and counterfactual fairness.
% CFGAN include two sets of generators and discriminators. 
% Discriminators in CFGAN integrate several types of causal fairness, such as total effect, direct or indirect discrimination and counterfactual fairness. 
\cite{Breugel2021DECAFGF} develop DECAF, a causally-aware GAN for generating fair synthetic data, and explicitly model the data generating process with an SCM in the input layers of the generator. 
% Compared to CFGAN, DECAF allows for post-hoc distribution changes of the synthetic data distribution, contributing to a flexible framework for selecting sensitive attributes. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/gan_prior_structure.pdf} 
    \caption{The illustration of encoding an SCM as the prior for latent variables in bidirectional generative models \protect\cite{shen2022weakly}.}
    \label{071106881268}
\end{figure}

\paragraph{\textbf{SCMs as a Prior for Latent Variables}}
In their study, \cite{shen2022weakly} propose a disentangled generative learning method that relaxes the requirement for careful hand-crafting in the translation of SCMs into generator networks. 
As shown in Figure \ref{071106881268}, this method integrates an SCM as the prior of a bidirectional generative model, such as BiGAN \cite{donahue2016adversarial}.  
A key difference from former studies is that \cite{shen2022weakly} only require causal variable labels, rather than specifying a complete causal graph. 
To represent the directed acyclic graph (DAG) $\mathcal{G}$, the study uses a weighted adjacency matrix $A$  and learns both the causal structure and assignments simultaneously through the use of general nonlinear function $f$ and $h$ for structural assignments.   
\begin{equation}
    \label{216591362718}
    z = f(({I-A^{\top}})^{-1} h(\epsilon))
\end{equation}
where $A$ is the weighted adjacency matrix and $\epsilon$ is exogenous noise variables. 
The authors aim to learn a disentangled causal representation in which underlying factors can be causally related, in contrast to existing disentanglement methods that assume a prior latent variable distribution with mutually independent components \cite{Locatello2019ChallengingCA}.
% This approach allows for more causal controllable generation and improved distributional robustness for downstream tasks. 
% Additionally, \cite{shen2022weakly} provide provable justification for the identifiability of the disentanglement due to the SCM prior and presents asymptotic convergence of the minimum loss.
It is important to note that the method proposed in \cite{shen2022weakly} utilizes a more direct and somehow stronger form of supervision in comparison to that of \cite{Khemakhem2020VariationalAA}.
Specifically, the method requires annotated labels of true factors to guarantee the identifiability of latent causal variables.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/internal_rep.pdf} 
    \caption{The illustration of the generative mapping and the intrinsic disentangled transformation in \protect\cite{Besserve2020CounterfactualsUT}.}
    \label{650437954687}
\end{figure}

\paragraph{\textbf{SCMs as Internal Representation}}
\cite{Besserve2020CounterfactualsUT} introduce the concept of intrinsic disentanglement as a way to perform interpretable and extrapolated transformation on data using a set of internal (endogenous) variables structured by an SCM. 
They argue that many disentanglement transformations are statistically dependent and unlikely to be disentangled in the latent space, and instead propose the use of modular parts of the network architecture (specifically, internal variables $v_1$ and $v_2$ as shown in Figure \ref{650437954687}) to ascribe properties to an image.
To do this, they use the channels $c$ of convolutional layers $l$ in deep generative models as initial interval variables, grouping these channels into modules using clustering algorithms based on the similarity of their influence maps.
Through experimentation, they validate the existence of these modules in various trained deep generative models and provide theoretical insights into how they can enable interpretable and extrapolated generations in pre-trained generative models \cite{Besserve2021ATO}.
% representing individual features like eyes, mouth, the background of the image or the hair.
% Thus, they choose initial interval variables as the collection of each channel $c$ of the output of a given convolutional layer $l$. Then, they group the channels into modules with clustering algorithms based on the similarity between influence maps. 
% such as Non-negative Matrix Factorization (NMF) and k-means
% Furthermore, experiments validate the existence of such modules of internal variables in various trained deep generative models. 
% They also provide theoretical insights into enabling extrapolated and interpretable generations for pre-trained generative models \cite{Besserve2021ATO}. 


% \begin{equation}
% \label{180326366387}
%     EIM(\xi) = \mathbb{E}_{z_2 \sim P(Z)} \mathbb{E}_{z_1\sim P(Z)} |Y_{v(z_2)}^{\xi}{(z_1)}-Y{(z_1)}|
% \end{equation}
% where $\xi = \{c\}$.



% Inspired by the causal principle of \textit{independent mechanisms} (IMs), they explore modularity in generative models, relaxing statistical independence in disentanglement learning. 
% \cite{Besserve2021ATO} develop a theory on the extrapolation issue in generative models based on causal independent mechanisms.

\subsubsection{GANs conform to SCMs}
Unlike the approach of explicitly encoding SCMs into structures of GANs, additional studies have explored more straightforward methods for downstream tasks, implementing generative strategies that follow the SCMs.

\paragraph{\textbf{Generative Intervention}}
% In such a manner, the model enables manufacture interventions and boosts the performance of tasks.
% Various studies propose utilizing the vanilla GANs directly and simultaneously enforcing the structural constraints within SCMs. 
In both \cite{Mao2021GenerativeIF} and \cite{Zhang2021LearningCR}, the use of GANs is utilized to simulate interventions based on an SCM.  
In the case of \cite{Mao2021GenerativeIF}, the goal is to improve the robustness of visual representations for downstream classification tasks. 
Since spurious correlations rarely exist beyond the training distribution, they analyze the causal relationships among stable and spurious features in visual classification tasks. 
Then this work utilizes conditional GAN (cGAN) \cite{Mirza2014ConditionalGA} to perform interventions on spurious variables. 
This procedure can also be interpreted as adversarial augmentation but under the constraint of interventions. 
The augmented data sampling with intervention possesses joint distributions that differ from the original observational data, thus eliminating spurious correlation and improving robust performance.   

Similarly, \cite{Zhang2021LearningCR} extend the concept of generative intervention to the realm of 3D pose estimation. 
They consider shifts in domains as interventions and conduct deep generative models to manufacture these interventions. 
The counterfactual features, in this case, belong to sample content, such as the person and object, but vary in terms of domain-specific information, such as background and viewpoint. 
Empirical validation presents that such transferable and causal representations contribute to the performance of 3D pose estimation tasks. 


\paragraph{\textbf{Knowledge Extrapolation}}
In order to bypass the limitations of using structural constructions corresponding to a causal graph with state-of-the-art GANs such as BigGAN \cite{Brock2019LargeSG}, \cite{Feng2022PrincipledKE} propose a method for generating counterfactual samples directly using pre-trained generators.
They assume that the extrapolation distribution only differs from the original distribution in the extrapolated knowledge dimension, which can be modeled through an adversarial game. 
This approach allows for greater flexible in integration with state-of-the-art GANs and results in the production of counterfactual results with high fidelity.



\subsection{VAEs-Based Models}
VAEs have been widely utilized for their ability to provide disentangled latent representations \cite{Kingma2014AutoEncodingVB}, and are considered a state-of-the-art in deep generative models \cite{Higgins2017betaVAELB}.
Several studies have posited that the latent variables within VAEs are mutually independent. 
This issue is closely aligned with nonlinear Independent Component Analysis (ICA), in which it is well-established that the generative procedure is not identifiable in the general nonlinear case. 
However, recent developments in this field \cite{Hyvrinen1999NonlinearIC,hyvarinen2019nonlinear} have demonstrated that if there are multiple distribution of the data that share the same generative function but have different distributions of the underlying independent latent variables, the generative function becomes identifiable \cite{Khemakhem2020VariationalAA,Kong2022PartialDF}.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth,height=2.5cm]{figures/illustration_pendulum.pdf} 
        \caption{The illustration of Pendulum dataset. 
        % The yellow object is light, and the red refers to a pendulum. 
        % As the light's position or pendulum's angle changes overtime, the black shadow also moves.
        }
        \label{019405822627}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.48\textwidth]{figures/causal_graph_pendulum.pdf} 
    \caption{The presumed causal graph.}
    \label{306104749773}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     % \hfill
%     \begin{subfigure}[h]{0.59\linewidth}
%         \includegraphics[width=\linewidth,height=2.5cm]{illustration_pendulum.pdf} 
%         \caption{The illustration of Pendulum dataset. 
%         % The yellow object is light, and the red refers to a pendulum. 
%         % As the light's position or pendulum's angle changes overtime, the black shadow also moves.
%         }
%         \label{019405822627}
%     \end{subfigure}
%     \hfill
%         \begin{subfigure}[h]{0.40\linewidth}
%         \includegraphics[width=\linewidth]{causal_graph_pendulum.pdf} 
%         \caption{The presumed causal graph.}
%         \label{792280998750}
%     \end{subfigure}
%     \caption{A swinging pendulum \protect\cite{Yang2021CausalVAEDR}. }
%     \label{238034286481}
% \end{figure}

\subsubsection{SCMs Integrated in VAEs}
% VAEs are commonly used to disentangle interpretable factorized representation from observational data \cite{Higgins2017betaVAELB}. 
% Since there is no formalized notion of disentangled representation,
In their work, \cite{Locatello2019ChallengingCA} define disentangled representation as the attempt to identify the distinct, semantic and informative factors of variations in the data.   
However, \cite{Yang2021CausalVAEDR} argue that in real scenarios, these factors of variations may not be only independent, as is commonly assumed in existing disentanglement approaches, but may also be causally related. 
As an example, when the light source or pendulum moves, the shadow's length and position also change, as shown in Figure \ref{019405822627}.
In order to address this issue, \cite{Yang2021CausalVAEDR} introduce CausalVAE, an approach to integrate an SCM into a vanilla variational autoencoder, as illustrated in Figure \ref{122145664592}.
% This is achieved through the use of an adjacency matrix to encode the causal relationships:
% \begin{equation}
%     \label{002914741521}
%     \mathbf{z} = \mathbf{A}^{\top} \mathbf{z} + \pmb{\epsilon} = (\pmb{I} -\mathbf{A}^{\top})^{-1} \pmb{\epsilon}, \pmb{\epsilon} \sim \mathcal{N}(0, \pmb{I})
% \end{equation}
% Additionally, the authors proposes a SCM layer,  as shown in Figure \ref{122145664592}, which allows for the propagation of causal effects between endogenous variables $z_i$:
% \begin{equation}
%     \label{460513906472}
%     z_i = g_i(\mathbf{A}_i \circ \pmb{z}; \pmb{\eta}_i)+\epsilon_i
% \end{equation} 
% where $g_i$ represents the mild nonlinear and invertible function that maps parental variables to the $z_i$ and $\mathbf{A}$ denotes an adjacency matrix to encode the causal relationships. 
% The proposed SCM layer enables the use of do-operation since when we intervene $z_i$, the causal effects could be propagated to itself and the descendant nodes according to Eq. (\ref{460513906472}).

It is worthnoting that the identifiablity \cite{Khemakhem2020VariationalAA} of CausalVAE is guaranteed through the utilization of surrogate information, specifically weak supervision of the labels on the latent causal variables of interest. 
CausalVAE can be seen as a pioneering study in the field \cite{shen2022weakly}, as it automatically learns causal structure through the use of adjacency matrices, which is distinct from that utilized in the CausalGAN \cite{Kocaoglu2018CausalGANLC}. 
% Additionally, the study provides theoretical guarantees for identifiability, following the work of \cite{Khemakhem2020VariationalAA}.
% When applied to the CelebA dataset, CausalVAE demonstrates the ability to learn causal semantic factors that can be intervened upon for counterfactual image generation.
Additionally, it should be noted, that CausalVAE implements a linear structural causal model with a maximum of four causal variables.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{figures/causalvae.pdf} 
    \caption{The model structure of CausalVAE, as depicted in  \protect\cite{Yang2021CausalVAEDR}, consists of a causal module and a SCM layer. The causal module utilizes an adjacency matrix to transform independent exogenous factors, represented by $\epsilon$, into causal representations. The SCM layer then reconstructs the causal representation $z$, simulating the transmission of causal effects. Additionally, the variables of interest are supervised by $u$.}
    \label{122145664592}
\end{figure}

\subsubsection{Estimate SCMs with VAEs}
In contrast to explicitly encoding SCMs, several studies have utilized VAEs to learn structural assignments \cite{Pawlowski2020DeepSC,Reinhold2021ASC,SnchezMartn2021VACADO}.   
Specifically, \cite{Pawlowski2020DeepSC} propose a novel deep generative framework called DeepSCM, which aims to infer counterfactual effects using a fully specified causal graph. 
They apply normalizing flow techniques and a VAE model to infer the exogenous noise variables related to endogenous variables and the structural assignments among causal variables. 
The complete SCM enables to perform a three-step causal procedure, namely abduction, action and prediction, providing a novel effective approach for answering causal questions. 
They extend the DeepSCM to model brain MRI scans images and present interesting and practical findings, whereas only present plausible counterfactual changes and lack quantifiable evaluations. 
However, this study is unable to account for unobserved confounders and operates under the assumption of causal sufficiency \cite{Scholkopf2022FromST}.

\cite{SnchezMartn2021VACADO} utilize graph neural networks (GNNs) to encode SCMs, as both belong to graph structures. 
They leverage Variational Graph Auto-Encoders (VGAE) and approximate the interventional effects using GNN message-passing algorithms. 
They represent the causal graph with an adjacency matrix embedded in each layer of the GNN, but also assume a known causal graph and the absence of hidden confounders.
However, the use of message aggregations in GNNs may limit the expressiveness and prevent it from handling larger causal graphs.  

In their work, \cite{Hu2021ACL} pivot the focus of text generations to a  causal perspective. 
Controllable text generation involves  generating texts that possess specific attributes and modifying samples to incorporate these attributes. 
This study, similar to DeepSCM \cite{Pawlowski2020DeepSC}, utilizes a VAE to infer exogenous variables and structural assignments among causal variables, despite examining various application domains. 




\subsection{Diffusion-Based Models}
\label{831281179594}

% Based on recent advances in diffusion probabilistic models \cite{Dhariwal2021DiffusionMB}, diverse studies unify generative diffusion models and SCMs for counterfactual estimation and explanations \cite{Sanchez2022DiffusionCM,Augustin2022DiffusionVC}. 
Recent research has demonstrated the potential for combining generative diffusion models and SCMs for counterfactual estimation and explanation through the use of diffusion probabilistic models \cite{Dhariwal2021DiffusionMB}. 
This approach has been explored in a number of studies \cite{Sanchez2022DiffusionCM,Augustin2022DiffusionVC}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/diffusion.pdf} 
    \caption{ The Diff-SCM model, which is a structured generative model, illustrates how the diffusion process can weaken the causal relationships between endogenous variables that are causally linked \protect\cite{Sanchez2022DiffusionCM}.}
    \label{802199783739}
\end{figure}

% Namely, an SCM $\mathcal{M}:=\{\mathbf{U}, \mathbf{X}, \mathcal{F}, P(\mathbf{U})\}$ comprises the components $X_1,\cdots,X_n$ of $\mathbf{X}$ as vertices in a DAG $\mathcal{G}$ whose arrows are represented by the structural assignments $f_i$ in $\mathcal{F}$, where $P(\mathbf{U})=\prod_{i=1}^N P(U_i)$ defines a joint distribution over mutually independent noise variables $\mathbf{U}$. Find the details of SCMs in \cite{Pearl2000CausalityMR,scholkopf2021toward,Scholkopf2022FromST,bareinboim2022pearl}. 

Namely, an SCM $\mathcal{M} := (\mathbf{S}, p(U))$ consists of structural assignments $\mathbf{S} = \{f^{(i)}\}_{i=1}^{K}$,
\begin{equation}
\label{052652870031}
    \mathbf{x}^{(k)} := f^{(k)}(\mathbf{pa}^{(k)}; \mathbf{u}^{(k)})
\end{equation}
where $\mathbf{x}^{(k)}$ represents the $k$-th known endogenous variable as a green node in Figure \ref{802199783739}; 
$\mathbf{pa}^{(k)}$ is the set of parents of $\mathbf{x}^{(k)}$ (its direct causes), such as $\mathbf{pa}^{(1)} = \{\mathbf{x}^{(2)}, \mathbf{x}^{(3)}\}$ in Figure \ref{802199783739};
$p(U) = \prod_{i=1}^{K}p(\mathbf{u}^{(k)})$ refers to a joint distribution over mutually independent exogenous noise variables.
Each $\mathbf{u}^{(k)}$ is only related to $\mathbf{x}^{(k)}$.
The joint distribution of endogenous variables can be decomposed using \textit{causal mechanisms}, represented by $p(\mathbf{x}^{(i)} \vert \mathbf{pa}^{(i)})$, rather than entangled factorizations, as implied by the  \textit{Causal Markov condition} in \cite{pearl2009causal,spirtes2000causation,scholkopf2021toward,Scholkopf2022FromST}:
% This is also known as \textit{Independent Causal Mechanism (ICM) Principle} \cite{scholkopf2021toward}, which states
\begin{equation}
\label{694530857668}
    p_{\mathcal{M}}(\mathbf{x}^{(i)},\cdots, \mathbf{x}^{(K)}) = \prod_{k=1}^{K} p(\mathbf{x}^{(k)} \vert  \mathbf{pa}^{(k)})
\end{equation}


\cite{Sanchez2022DiffusionCM} propose Diff-SCM as a way to unite SCMs and the stochastic differential equation (SDE) framework \cite{Song2021ScoreBasedGM,weng2021diffusion}.
As depicted in Figure \ref{802199783739}, they formulate a forward diffusion as a process of weakening the causal relations between endogenous variables.
Specifically, the original joint distribution entailed by the Eq. (\ref{694530857668}) that diffuses to independent Gaussian distributions $p(U)$, as  $p(\mathbf{x}_{t=T}^{(k)}) = p(\mathbf{u}^{(k)})$ and $p(\mathbf{x}_{t=0}^{(k)}) = p_{\mathcal{M}}(\mathbf{x}^{(k)})$ with $t \in [0, T]$.
Following the time-dependent SDE \cite{Song2021ScoreBasedGM}, Diff-SCM is defined as:
\begin{equation}
\begin{aligned}
    \label{143892833217}
    d\mathbf{x}^{(k)} &= -\frac{1}{2} \beta_{t} \mathbf{x}^{(k)} dt + \sqrt{\beta_t}d\mathbf{w}, \forall k \in [1, K], \\
    \text{where}\   p(&\mathbf{x}_{0}^{(k)}) = \prod_{j=k}^{K} p(\mathbf{x}^{(j)} \vert \mathbf{pa}^{(j)}), p(\mathbf{x}_T^{(k)}) = p(\mathbf{u}^{(k)})
\end{aligned}
\end{equation}
where $\beta_t \in [0,1]$ represents the time-dependent variance of a Gaussian noise introduced in each forward process and $\mathbf{w}$ is the Brownian motion leading to a Gaussian distribution.  

This study utilizes an anti-causal predictor inspired by the classifier-guided diffusion introduced in previous work \cite{Dhariwal2021DiffusionMB}.
This approach involves transforming the prior distribution $p(U)$ into the data distribution through a gradual removal of noise using the gradient of the data distribution, until $\mathbf{x}_{t=0}^{(k)} = \mathbf{x}^{(k)}_{}$ (as described in \cite{Song2021ScoreBasedGM}).
With the aim of achieving conditional generation, \cite{Dhariwal2021DiffusionMB} train a classifier and use its gradients to guide the diffusion process towards the desired conditioning information.
To obtain counterfactual samples, they pass the gradients of the predictor through a reverse-diffusion process after performing an intervention (assigning a specific value to the cause).
These counterfactual samples are highly similar images that differ only in their class label.
This work follows three steps of causal hierarchy, similar to \cite{Pawlowski2020DeepSC}, but is limited to a bi-variable SCM with the causal relationship $\mathbf{x}^{(2)} \rightarrow \mathbf{x}^{(1)}$, where $\mathbf{x}^{(1)}$ represents an image, $\mathbf{x}^{(2)}$ represents a class label.

% The original generative process in the SDE is done by transforming the prior distribution $p(U)$ into the data distribution by slowly removing the noise \cite{Song2021ScoreBasedGM} with the gradient of the data distribution, until $\mathbf{x}_{t=0}^{(k)} = \mathbf{x}^{(k)}_{}$. 
% Aiming for conditional generations, \cite{Dhariwal2021DiffusionMB} train a classifier and use the gradients to guide the diffusion process towards the conditioning information.
% \cite{weng2021diffusion}.
% Inspired by such classifier-guided diffusion, this study explores an anti-causal predictor \cite{Schlkopf2012OnCA,Kilbertus2018GeneralizationIA} to guide the generative process. 
% For simplicity, the terminology of anti-causal refers 
% After an intervention is performed (the cause is assigned with a specific value), the counterfactual samples would output by passing the gradients of the predictor to the reverse-diffusion process. 
% Counterfactual samples here refer to images that are highly similar but differ in the class label.


% \begin{equation}
% d \mathbf{x}^{(k)} = [-\frac{1}{2} \beta_t + \beta_t \nabla_{\mathbf{x}_t^{(k)}} log p_{\mathcal{M}}(\mathbf{x}^{(j)} = x^{(j)} \vert x_{t}^{(k)})] dt + \sqrt{\beta_t} \tilde{\mathbf{w}}
% \end{equation}


% Analogously to \cite{Pawlowski2020DeepSC}, \cite{Sanchez2022DiffusionCM} take three steps for counterfactual estimation with a deep generative learning perspective as well. 
% The three steps comprise (i) abduction of exogenous noise by the forward diffusion process with the denoising diffusion implicit model \cite{Song2021DenoisingDI}; (ii) action with graph mutilation by erasing the edges between the intervened variable and its parents; (iii) prediction with reverse diffusion process controlled by the gradients of an anti-causal classifier. 
% To the best of our knowledge, this study, named Diff-SCM, is the first work that integrates recent advances in diffusion models and structural causal models. 
% They build an simplified SCM with two variables: $\mathbf{x}^{(1)}$ stands for an image and $\mathbf{x}^{(2)}$ represents a class.   
% They simulate interventions on the class label $\mathbf{x}^{(2)}$, achieving qualitatively and quantitatively high similarity with each counterfactual and only differing in the class label.  


Subsequently, \cite{Sanchez2022WhatIH} improve the Diff-SCM by introducing implicit attention guidance for lesion segmentation. 
Given an input image, the authors synthesize healthy counterfactual images by making minimal changes to the input but altering the domain. 
The difference between the original patient image and the healthy counterfactual is used to create a heatmap that indicates the location of the pathology. 
By using implicit attention guidance in the counterfactual diffusion probabilistic model (CDPM) rather than a downstream classifier, they demonstrate the superior performance of their approach. 
Other research has also explored the use of diffusion models for generating counterfactual images and providing counterfactual explanations (CEs) \cite{Goyal2019CounterfactualVE,Augustin2022DiffusionVC}. 
% This paper \cite{Sanchez2022WhatIH} investigates a question of "How would a patient appear if X pathology was not present?". 
% \cite{Goyal2019CounterfactualVE} formulate a description of CEs as the following: given a target class $c$ and a query image $X$, a counterfactual explanation identifies what is the minimal change $\delta$ of input $X$, such that the system would output a different class $c^{\prime}$ for $X+\delta$. In order to generalize to classificatio problems with arbitrary classes, 
% \cite{Augustin2022DiffusionVC} attach two key modifications to the diffusion process: an adaptative parameterization and the cone regularization via an adversarially robust model.





% \cite{khemakhem2021causal}

==> tables/taxonomy.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    % line width=0.8pt,
]
\tikzstyle{leaf}=[
    my-box, 
    minimum height=1.5em,
    % fill=hidden-orange!60, 
    fill=hidden-blue!90, 
    text=black,
    align=left,
    font=\normalsize,
    % font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
    % line width=0.8pt,
]
\begin{figure*}[th!]
    \vspace{-2mm}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            % forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-black,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=10.5em,font=\normalsize,}{},
            where level=2{text width=13.5em,font=\normalsize,}{},
            where level=3{text width=12em,font=\normalsize,}{},
            % where level=4{text width=12em,font=\normalsize,}{},
            [
                Deep Learning \\ Methods
                [
                    Neural Networks (\S )
                    [
                        Seq2Seq-based  (\S )
                        [
                            \eg DNS~{,}
                            AnsRat~
                            , leaf, text width=32em
                        ]
                    ]
                    [
                        Seq2Seq-based  (\S )
                        [
                            \eg DNS~{,}
                            AnsRat~
                            , leaf, text width=32em
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    % \vspace{-4mm}
    \caption{Taxonomy of deep learning for mathematical reasoning.}
    \label{fig:taxonomy}
    % \vspace{-3mm}
\end{figure*}
